Length Generalization in Arithmetic Transformers

We examine how transformers cope with two challenges: learning basic integer arithmetic, and generalizing to longer sequences than seen during training. We find that relative position embeddings enable length generalization for simple tasks, such as addition: models trained on $5$-digit numbers can perform $15$-digit sums. However, this method fails for multiplication, and we propose train set priming: adding a few ($10$ to $50$) long sequences to the training set. We show that priming allows models trained on $5$-digit $\times$ $3$-digit multiplications to generalize to $35\times 3$ examples. We also show that models can be primed for different generalization lengths, and that the priming sample size scales as the logarithm of the training set size. Finally, we discuss potential applications of priming beyond arithmetic.

==> mathcommands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newcommand{\gen}{\mathcal{G}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\integers}{\mathbb{N}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\erf}{\mathrm{erf}}
\newcommand{\EE}{\mathbb{E}\,}
\newcommand{\DKL}[2]{\ensuremath{D\left( #1 \, \|  \, #2 \right)}}
\newcommand{\DeltaKL}{\ensuremath{\Delta_\mathrm{KL}}}
\newcommand{\DeltaW}{\ensuremath{\Delta_{W^2}}}
% some further math short-hands
\newcommand{\cN}{{\cal N}}
\newcommand{\usD}{\frac{1}{D}}
\newcommand{\ussD}{\frac{1}{\sqrt{D}}}
\newcommand{\ussdelta}{\frac{1}{\sqrt{\delta}}}
\newcommand{\usN}{\frac{1}{N}}
\newcommand{\ussN}{\frac{1}{\sqrt{N}}}
\newcommand{\dd}{\operatorname{d}\!}
\newcommand{\bs}{\boldsymbol}

\usepackage{xcolor}
\definecolor{C0}{HTML}{1f77b4}
\definecolor{C1}{HTML}{ff7f0e}
\definecolor{C2}{HTML}{2ca02c}
\definecolor{C3}{HTML}{d62728}
\definecolor{C4}{HTML}{9467bd}
\definecolor{C5}{HTML}{8c564b}
\definecolor{C6}{HTML}{e377c2}
\definecolor{C7}{HTML}{7f7f7f}
\definecolor{C8}{HTML}{bcbd22}
\definecolor{C9}{HTML}{17becf}

\newcommand{\ntrain}{n_\text{train}}
\newcommand{\ntest}{n_\text{test}}


==> num_exp.tex <==
\section{Numerical experiments}

\subsection{Addition}

\begin{figure}[tbp]
\vspace*{-1.5cm}
\begin{subfigure}{0.32\textwidth}
\centering
` \includegraphics[width=1\linewidth]{images/albert_addition_attention_heads.pdf}
%  \vspace{-8mm}

  \vspace{-2mm}
\caption{}\label{fig:albertheads}
\end{subfigure}
%\hspace*{1cm}
\begin{subfigure}{.32\textwidth}
\includegraphics[width=1\linewidth]{images/albert_addition_hiddensize.pdf}
\vspace*{-7mm}
\caption{}\label{fig:alberthidden}
\end{subfigure}
\begin{subfigure}{.32\textwidth}
\includegraphics[width=1\linewidth]{images/albert_addition_depth.pdf}
\vspace*{-7mm}
\caption{}\label{fig:alberthidden}
\end{subfigure}
\caption{Scaling laws for addition}
\end{figure}









\subsection{Multiplication}

\begin{figure}[tbp]
\vspace*{-1.5cm}
\begin{subfigure}{0.24\textwidth}
\centering
 \includegraphics[width=1\linewidth]{images/albert_minsamples_3digits.pdf}
%  \vspace{-8mm}

  \vspace{-2mm}
\caption{}\label{fig:albertmultlongseq}
\end{subfigure}
%\hspace*{1cm}
\begin{subfigure}{.24\textwidth}
\includegraphics[width=1\linewidth]{images/albert_15x3_samples.pdf}
\vspace*{-7mm}
\caption{}\label{fig:shortseq}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
\includegraphics[width=1\linewidth]{images/ALBERT3000samples_time.pdf}
\vspace*{-7mm}
\caption{}\label{fig:complexitysample}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
\includegraphics[width=1\linewidth]{images/hist_ood_albert3000.pdf}
\vspace*{-7mm}
\caption{}\label{fig:digitextrapolation}
\end{subfigure}
\caption{Length generalization with a transformer trained on 5x3 multiplication. (a) shows the number of long sequences that is needed to get successful extrapolation for varying length integers. (b) shows how the OOD accuracy varies as we increase the number of long sequences. (c) shows how the ID and OOD accuracies vary as we increase the number of short sequences. (d) Final accuracy obtained on varying length integers. }


\textcolor{red}{ Maybe a plot to show how when we do not add data, nothing changes}

\end{figure}



\begin{itemize}
   \item[--] Addition experiments: take HL = 4, HS = 1024, AH = 16
   \begin{itemize}
      \item[$\ast$] try BERT, ALBERT with fixed and relative positional encoding (vary length generalization)
   \end{itemize}
   \item[--] Multiplication experiments: 
   \begin{itemize}
      \item[$\ast$] RPE, ALBERT and scaling all the params (HS, HL and AH) still 0 OOD but 100 ID
      \item[$\ast$] Change plot (a) to put percentage of data that is needed.
      \item[$\ast$] instead of putting 10\% like in the 3k, let's try 50\%. Do we get better buckets in (d)?
      \item[--] let's put 5\% of of 20 and 5\% of 10 in the 3k exp. Do we generalize to everyone (exp Fig. 2d)?
      \item[$\ast$] Fine-tuning does not work? curriculum where we increase number of data?
      \item[$\ast$] 50\% of 5 and 50\% of 20: Fig 2 (c). Which one goes faster?
      \item[$\ast$] 10, 12 and 
   \end{itemize}
\end{itemize}

==> old_intro_llm.tex <==
\section{Introduction}


Since the advent of Transformers~\cite{vaswani2017attention}, large language models (LLMs), sometimes called foundation models, have become the forefront of Natural Language Processing, for the better and the worst~\cite{bommasani2021opportunities}. Blessed with the power of scaling laws~\cite{kaplan2020scaling}, these models have since grown  tenfold in size every year, and are currently reaching the bar of a trillion parameters. 


State-of-the-art models such as GPT-3~\cite{brown2020language} display impressive text generation abilities, and also exhibit rather impressive abilities when prompted a few examples. Nonetheless, these models fail in very simple reasoning tasks such as \emph{learning arithmetic}. In this task, the model has access to arithmetic operations either during training time or in-context and then predicts the output of unseen operations at evaluation time. This task is challenging as the model needs to parse the input, identify the appropriate digits, apply a rule, store the result of these intermediate steps and finally recombine them.  Even in the in-distribution 
(ID) setting where the integers are sampled from the same distribution at training and evaluation time, the test accuracy is low \citep{anil2022exploring}. 


\fc{Not just LLM: small transformers, and other sequential models struggle with arithmetic.

I think we should explain that there are two problems: plain arithmetic, and out of distribution generalization. 
}

Recently, several works \cite{nye2021show,wei2022chain,lewkowycz2022solving} proposed to use a scratchpad, or chain-of-thought reasoning, when prompting LLMs. In addition of the standard inputs and label that are given to the model, we break down the task  into multiple small steps and provide
these steps. Using this concept, several papers showed that LLMs achieve in-distribution generalization in arithmetic \cite{nye2021show,zhou2022teaching}. 

However, it remains open whether LLMs with scratchpad understand the mechanism behind these arithmetic operations. For this reason, \cite{nye2021show} and \cite{zhou2022teaching} have considered a more robust evaluation measure which is  \emph{length generalization}: at training/in-context time, the model is given integers of length at most $\ntrain$ and is then evaluated  on  integers of length $\ntest>\ntrain.$ Ideally, if the model has really learnt the arithmetic rule, then the length of the integers should not influence its performance. Both \cite{nye2021show} and \cite{zhou2022teaching} show that scratchpad gives non-trivial performance but is insufficient for length generalization. Recently, \cite{zhou2022teaching} proposed to improve scratchpad through algorithmic prompting. This technique consists in teaching the LLM an arithmetic operation by providing  a detailed description of the underlying algorithm 
on running examples. While the length performance of their LLMs is impressive on addition operations, their approach presents a few drawbacks: first, it requires tailored prompts for each operation  which may be limited. More importantly, designing the appropriate prompt for a given operation may be very hard in that they may be very long and hard to formalize. For instance, in the case of multiplication, the prompt is quite long and the model is only able to length generalize to 3-digit multiplication. 




In this paper, we address the length generalization of LLMs in arithmetic from a different standpoint. We start from a \emph{randomly initialized} LLM, train it with integers of length $\ntrain$ and then evaluate it on integers of length $\ntest.$ By leveraging  techniques detailed below, we show that LLMs are able to length generalize in addition, modular addition and multiplication.  More precisely, we
make the following contributions:
\begin{itemize}[leftmargin=*, itemsep=1pt, topsep=1pt, parsep=1pt]
\item[--] In \autoref{sec:setting}, we present the numerical setup. We describe how the data is generated and formatted; the training and evaluation procedures; and the models that we train.
\item[--] In \autoref{sec:addition}, we show that off-the-shelf BERT-like encoders \cite{devlin2018bert} length generalize in the case of addition. We distinguish three ingredients for successful extrapolation: relative positional embeddings, shared layers as in ALBERT \cite{lan2019albert} and model scaling.
\item[--] In \autoref{sec:multiplication}, we first show that the techniques used in the  addition case do not translate to the multiplication setting. We then show that when  \emph{few-shot training} an LLM --which consists in training a model on a training set mostly made of short integers and a tiny amount of long integers, the model length generalizes on large test datasets. To our knowledge, this paper is the first showing that a deep learning model can length generalize to very long integers multiplication.
\end{itemize}

\paragraph{Key messages.} This paper advocates for few-shot training Transformers in order to length generalize in multiplication. We highlight the following observations:
\begin{itemize}[leftmargin=*, itemsep=1pt, topsep=1pt, parsep=1pt] 
   \item[$\ast$] \textbf{Fine-tuning fails}: when fine-tuning the model, we observe that the performance on the short sequences decays (catastrophic forgetting), while the performance on the long sequences first increases and eventually decreases. 
   \item[$\ast$] \textbf{Amount of few-shot examples barely increases with training size}: given a training set with $\Ntrain$ examples where we we add $\Ntest$ long integers, we show that $\Ntest$ varies logarithmically with $\Ntrain$. Thus, even with gigantic training sets, a tiny amount of few-shot examples is needed.
   \item[$\ast$] \textbf{Transformer understands the rule}: when adding examples with $\ntest$ and $(\ntest-1)$-length integers, the model predicts the correct result  faster and with higher accuracy than a model only trained with $\ntest$-digits integers. Thus, the model uses its knowledge from the shorter sequences to length generalize. 
   \item[$\ast$] \textbf{Curricula fail in few-shot training}: given a data budget $\Ntest$ of long integers, what is the best allocation among all the possible long integers to reach high accuracy on $\ntest$-digit integers? The optimal strategy is to allocate all the budget on $\ntest$-digit integers and curricula that consist in training with intermediate length integers fail.
   \item[$\ast$] \textbf{Generalization to intermediate lengths}: adding $\ntest$-digit integers to the training set yields to generalization on $\ntest$-digit integers. However, the model poorly generalizes on $\nval$-digit integers with $ \ntrain<\nval< \ntest$.  Adding $\Ntest$ $\nval$-examples for each $\nval$ in the training dataset yields length generalization for all the intermediate length integers.
\end{itemize}

 

%bcp de modele sont des problemes. il y a un probleme de generalisation aux plus petites/longueurs. few-shot methode principale. d'une part juste en RPE. Pour des pb plus compliques, RPE ne marche pas. On montre que rajouter qqs elements marche. Optimisation des distribtuon nous aide. On montre que ca marche pour d'autres modeles.


==> old_introduction_jan19.tex <==
\section{Introduction}

%Transformers are deep learning models built on self-attention  \citep{vaswani2017attention}, and in the past several years they have increasingly formed the backbone for state-of-the-art models in domains ranging from Natural Language Processing (NLP)  \citep{vaswani2017attention,devlin2018bert} to computer vision \citep{dosovitskiy2020image}, reinforcement learning \citep{chen2021decision,janner2021offline}, and program synthesis \citep{austin2021program}. %This motivates their use in more challenging settings such as reasoning tasks \cite{cobbe2021training,hendrycks2021measuring}. %, and trained models have difficulty to generalize to numbers larger than those seen during training \cite{zhou2022teaching}
%Despite their successes, Transformers still struggle on deceptively simple tasks. Arithmetic is one such example: whereas Transformers can be trained to perform addition \cite{nogueira2021investigating}, multiplication of large numbers proves hard to learn. This inability to perform basic arithmetic has been observed in recent large language models (which are transformer based) such as ChatGPT \citep{schulman2022chatgpt} and is partly responsible for the failures of these large-scale models to perform reasoning, and solve problems of science. Alleviating these shortcomings is thus key to build reasoner models. Besides, from a scientific perspective, arithmetic is appealing in that it is a  controllable setting. Contrary to computer vision and NLP, we can measure the hardness of an example, e.g., an addition instance which involves computing multiple successive carries is difficult, and have a better understanding of what the model learns.
%, where they can perform addition \cite{nogueira2021investigating} but struggle with multiplication of large numbers.

Transformers are deep learning models \citep{vaswani2017attention} that have achieved remarkable results in domains ranging from Natural Language Processing (NLP) \citep{vaswani2017attention,devlin2018bert}, computer vision \citep{dosovitskiy2020image}, reinforcement learning \citep{chen2021decision,janner2021offline}, and program synthesis \citep{austin2021program}. However, they still face challenges in seemingly simple tasks such as  arithmetic. This inability to perform basic arithmetic has been observed in recent large language models (which are transformer based) such as ChatGPT \citep{schulman2022chatgpt} and is partly responsible for the failures of these large-scale models to perform reasoning, and solve problems of science. Enhancing their arithmetic capabilities is thus essential for developing better reasoner models. %Additionally, arithmetic provides a suitable setting for scientific exploration, where we can assess the hardness of an example, e.g., by measuring the number of carries required in an addition problem, and gain more insight into what the model learns.
 
 
A long line of works has explored the capacity of machine learning models to learn arithmetic. Initial works focused on recurrent architectures such as Neural GPUs \citep{kaiser2015neural} or LSTMs \citep{palamas2017investigating,saxton2019analysing}. Subsequently, researchers examined the use of Transformers  
\cite{nogueira2021investigating,power2022grokking} to learn addition and modular operations. \citet{ling2017program} proposed a hybrid solution where the Transformer could call an external calculator to perform arithmetic.  These works are in the in-distribution (ID) case where the integers in the training and test sets are drawn from the same distribution. However, this setup does not reflect what we would expect from a model that learns arithmetic. Indeed, when humans learn two-digits numbers addition, they can apply the same method to numbers of \emph{arbitrary length}. Similarly, an ideal  Transformer should learn the underlying algorithm in an arithmetic operation and not memorize the answers from a limited range of inputs.

%objective of learning arithmetic, which is to perform arithmetic operations on \emph{any input size}. For example, humans can learn how to add two-digit numbers and then apply the same method to numbers of arbitrary length.
%\citet{nogueira2021investigating} underline the difficulty of learning addition with Transformers and show that the representation of the numbers given to the model is critical for high test accuracy
 
 In this regard, out-of-distribution (OOD) generalization measures such as \emph{length generalization} better reflect the understanding of the model. In this framework, the network is trained on integers of length at most $\ntrain$ and then evaluated  on  integers of length $\ntest>\ntrain.$ Ideally, if the model has learnt the arithmetic rule, then the length of the integers should not impact its performance. To our knowledge, \citet{trask2018neural} is the only work that achieved this extrapolation using randomly initialized models. They design NALU, an architecture that learns addition and multiplication and generalize to any value. However, their network have hand-crafted modules that are specifically designed to encode addition and multiplication. Thus, the model does not manage to perform arithmetic because it has learnt it but rather because it was encoded. Achieving length generalization remains a challenge for Transformers that is caused by the position embedding (PE) method and several works proposed to either modify it \cite{raffel2020exploring,su2021roformer} or to replace it by weighted local attention \cite{press2021train}. However, these works are limited to NLP tasks and it remains open whether they are effective in arithmetic.


%In this paper, we investigate the capability of Transformers to learn arithmetic, by learning to translate a pair of operands into their sum, modular sum, or product. In particular, we evaluate, on these three tasks, the ability to generalize to operands larger than those seen during training.


%In this paper, we consider one of these tasks which is \emph{learning arithmetic} wherein the input consists of  two integers and an operator and its corresponding label is the result of this operation. After training a model on a dataset made of such operations, the model must predict the output of unseen operations at evaluation time. This task is challenging as the model needs to parse the input, divide the task into subproblems, apply a rule, store the result of these intermediate steps and finally recombine them. \textcolor{red}{Arithmetic is also attractive from a scientific perspective since we can control the complexity of the tasks, identitfy the hard cases, probe specific abilities of the model and so on.}





%\fc{ \citet{trask2018neural} proposed NALU, networks with constrained weight values, that can learn addition and multiplication and generalize to any value. However, their extension to division, modular operations and more complex calculations seem difficult. Generalization to longer sequences than those seen during training is a known limitation of the original transformer. It seems to originate in the use of position embedding (PE). Several mitigations have been proposed: relative position embeddings, replacing the PE by weighted local attentions (cite ALIBI by Press). Retraining techniques, like few-shot learning have also been considered. }







%Aforementioned works are in the in-distribution (ID) case where the numbers at training and test times are sampled from the same distribution. This setting may be misleading as the model may get high test accuracy and yet, miss the key steps of the mechanism behind these arithmetic operations. Similarly to \cite{nye2021show} and \cite{zhou2022teaching}, we consider a more robust evaluation measure which is  \emph{length generalization}:  the model is trained on integers of length at most $\ntrain$ and is then evaluated  on  integers of length $\ntest>\ntrain.$ Ideally, if the model has learnt the arithmetic rule, then the length of the integers should not impact its performance.

% In this paper, we investigate the capability of Transformers to learn arithmetic, by learning to translate a pair of operands into their sum, modular sum, or product. In particular, we evaluate, on these three tasks, the ability to generalize to operands larger than those seen during training.

 In this paper, we investigate the capability of Transformers to learn arithmetic, by learning to translate a pair of operands into their sum, modular sum, or product.  
We show that by leveraging some tricks detailed below, Transformers are able to length generalize in these three tasks.  More precisely, we
make the following contributions: 
\textcolor{red}{Insist that we do on 35.} 


\begin{itemize}[leftmargin=*, itemsep=1pt, topsep=1pt, parsep=1pt]
\item[--] In \autoref{sec:setting}, we present the numerical setup. We describe the data generation and format; the training and evaluation procedures; and the models that we train.
\item[--] In \autoref{sec:addition}, we show that BERT-like encoders \cite{devlin2018bert} can length generalize in the case of addition. We distinguish two ingredients for successful extrapolation: data padding and relative position embeddings. We show that using shared layers as in ALBERT \cite{lan2019albert} and scaling the model lead to improved results.
\item[--] In \autoref{sec:multiplication}, we first show that the techniques used for addition case are not successful in the multiplication setting. We then show that when  \emph{few-shot training} an LLM, i.e.\  training a model on many instances with short integers and adding a tiny amount of long integers instances, the model length generalizes. To our knowledge, this paper is the first showing that a Transformer can length generalize to multiplication of very long integers.
\end{itemize}

%The length generalization setting assumes that we train a model on $\Ntrain$ examples with operations on $\ntrain$-digits integers. We then evaluate on $\ntrain$-digits instances where $\ntest > \ntrain.$ 

\paragraph{Key messages.}  
We advocate for few-shot training Transformers in order to length generalization on multiplication. This technique consists in training with  $(\Ntrain-\varepsilon)$ examples having $\ntrain$ digits and adding few-shot examples i.e.\ $\varepsilon$ instances with $\ntest$ digits where $\varepsilon \ll \Ntrain$. We emphasize the following observations:
\begin{itemize}[leftmargin=*, itemsep=1pt, topsep=1pt, parsep=1pt] 
   \item[$\ast$] 
   \textbf{Standard training fails}: when only training on $\ntrain$-digit integers, extrapolation to longer sequences is not possible even in very simple cases
   (\autoref{fig:heatmap_mul}) and using relative embeddings does not fix the problem.%such as ALIBI \citep{press2021train} does not fix the problem \textcolor{red}{Exp with ALIBI}.
   \item[$\ast$] \textbf{Fine-tuning is sample-expensive}: when training on short sequences and fine-tuning on long ones, we observe  two limitations. First, we observe that the performance on the short sequences decays to zero even after a few optimization steps (catastrophic forgetting). Besides, the number of few-shot examples required to length generalize must be large (\textcolor{red}{Figure ***}).
   \item[$\ast$] \textbf{Amount of few-shot examples barely increases with training size}: we show that the number of few-shot examples is very small compared to the training size even for challenging multiplications (\autoref{fig:fewshot}). Besides, as we increase $\Ntrain$, we observe that $\varepsilon$ grows logarithmically (\autoref{fig:fewshot_trainingsize}). Thus, on gigantic training sets, a tiny amount of few-shot examples is needed.
   \item[$\ast$] \textbf{Optimal allocation of few-shot examples}: given a few-shot budget $\varepsilon$, what is the best allocation among all the integers to reach high accuracy on $\ntest$-digit integers? The optimal strategy is to allocate all the budget on $\ntest$-digit integers. Assigning some budget to intermediate length integers does not yield better accuracy.
   \item[$\ast$] \textbf{Model understands some logic in multiplication}: when adding few-shot examples examples with $n$ ( $n\in(\ntrain,\ntest)$) and $\ntest$ digits, does the model use the intermediate-length examples to learn the long sequence multiplications? We add $\ntest$ and $(\ntest-1)$-length integers to the training set and the model gets faster and higher accuracy than when trained on $\ntest$-digit integers (\autoref{fig:understandmul}). 
   \item[$\ast$] \textbf{Generalization to intermediate lengths}: with few-shot training,   the model poorly generalizes on $n$-digits integers for $n\in (\ntrain,\ntest)$ (\autoref{fig:hist_vanilla}). However, when we add $\varepsilon$ few-shot examples for each $n$, we obtain length generalization to all the intermediate lengths.
\end{itemize}

 

%bcp de modele sont des problemes. il y a un probleme de generalisation aux plus petites/longueurs. few-shot methode principale. d'une part juste en RPE. Pour des pb plus compliques, RPE ne marche pas. On montre que rajouter qqs elements marche. Optimisation des distribtuon nous aide. On montre que ca marche pour d'autres modeles.


==> todo.tex <==
\section{TODO list}


\begin{itemize}
   \item[--] Addition: try absolute positional encodings and show it fails. 
   \item[--] Multiplication: different ideas to dig into. 
   \begin{itemize}
      \item[$\ast$] \textbf{Training size vs number of examples}: Try different training sizes TS (1e3, 5e3, 1e4, 5e4, 1e5, 5e5) and show that the needed number of samples vary like $c\cdot \log(\text{TS}/\text{digit number})$. 
      \item[$\ast$] \textbf{Fill the buckets}: add 50 samples from 10 to 35 and see whether it learns all the numbers there? 
      \item[$\ast$] \textbf{Short sequences help}: I put 50 samples on 35 vs 50 samples on 33, 34 and 35. Do I have faster convergence to 35 length? Do I have higher accuracy on 35? 
      \item[$\ast$] \textbf{Curricula schemes fail}: let's say that the minimum that works is 50 samples on 5k. Imagine I split the 50 uniformly in (34,35), (32,33,34,35), \dots. 
      Try increasing, decreasing (linear, quadratic, exponential).
      \item[$\ast$] \textbf{Fine-tuning fails}: take a model that is trained on 5 digits and fine-tune it on 6. Show that actually, performance of 5 decays and on 6 it increases then decreases. Catastrophic forgetting.
      \item[$\ast$] Look at multi-operand generalization?
      \item[--] Modular addition: show that fine-tuning fails even on 6 and show few-shot training works.
   \end{itemize}
\end{itemize}


bcp de modele sont des problemes. il y a un probleme de generalisation aux plus petites/longueurs. few-shot methode principale. d'une part juste en RPE. Pour des pb plus compliques, RPE ne marche pas. On montre que rajouter qqs elements marche. Optimisation des distribtuon nous aide. On montre que ca marche pour d'autres modeles.

section 2: problemes mathematiques que tu regardes, modeles, 


section 3: resultats experiments
